A Finite-Difference Time-Domain approach for dispersive magnetic media

We extend the Finite-Difference Time-Domain method to treat dispersive magnetic media by incorporating magneto-optical effects through a frequency-dependent permittivity tensor. For benchmarking our method, we consider the light scattering on a magnetic sphere in the Mie regime. We first derive the analytical scattering expressions which predict a peak broadening in the scattering efficiency due to the atomic energy level splitting in the presence of a magnetic field, together with an additional rotated part in the scattered field profile due to the Faraday rotation. We show that our numerical method is able to capture the main scattering features and discuss its limitations and possible improvements in accuracy.

==> FDTD for magnetic dielectrics - arxiv/sub.tex <==
% \documentclass{optica-article}

% \journal{opticajournal} % for journals or Optica Open

% \articletype{Research Article}

% \usepackage{lineno}
% \linenumbers % Turn off line numbering for Optica Open preprint submissions.

% \usepackage{siunitx}

% \newcommand{\Heff}[1]{\boldsymbol{H}_{\rm eff}\left[#1\right]}



% \begin{document}

% %##############################################################

\title{Supplemental material}

% %##############################################################
\section{Light scattering on a magnetic sphere}
In the following we provide additional derivations for the light scattering on a magnetic sphere as discussed in the main text.

%Field expansion
\subsection{Field expansion}
\label{sup:expansion}
All electromagnetic fields $\boldsymbol{\mathbf{F}} \in \{ \boldsymbol{\mathbf{E}}, \boldsymbol{\mathbf{B}}, \boldsymbol{\mathbf{D}}, \boldsymbol{\mathbf{H}}\}$ can be expanded as
\begin{equation}
    \boldsymbol{\mathbf{F}} (\boldsymbol{\mathbf{r}}) = \sum_{lm} \frac{1}{r} \left[ \mathcal{F}_{lm}^X(r) \boldsymbol{\mathbf{X}}_l^m (\theta, \phi) + \mathcal{F}_{lm}^Y(r) \boldsymbol{\mathbf{Y}}_l^m (\theta, \phi) + \mathcal{F}_{lm}^Z(r) \boldsymbol{\mathbf{Z}}_l^m (\theta, \phi) \right],
    \label{eq:expansion}
\end{equation}
where $\mathbf{R}_l^m$ are the vector spherical harmonics given by
\begin{equation}
    \begin{split}
        \boldsymbol{\mathbf{X}}^m_l(\theta, \phi) &= Y^m_l(\theta, \phi) \, \hat{\boldsymbol{\mathbf{r}}}, \\[0.2cm]
        \boldsymbol{\mathbf{Y}}^m_l(\theta, \phi) &= \frac{1}{\sqrt{l(l+1)}} \, \mathbf{L} \, Y^m_l(\theta, \phi) \\[0.2cm]
       &=  \frac{i}{\sqrt{l(l+1)}} \left[ \frac{1}{\sin \theta} \, \partial_{\phi} Y^m_l(\theta, \phi) \, \hat{\boldsymbol{\theta}} -  \partial_{\theta} Y^m_l(\theta, \phi) \, \hat{\boldsymbol{\phi}} \right] , \\[0.2cm]
        \boldsymbol{\mathbf{Z}}^m_l(\theta, \phi) &= \frac{ir}{\sqrt{l(l+1)}} \, \boldsymbol{\nabla} Y^m_l(\theta, \phi)  \\[0.2cm]
        & = \frac{i}{\sqrt{l(l+1)}} \left[ \partial_{\theta } Y^m_l(\theta, \phi) \, \hat{\boldsymbol{\theta}} + \frac{1}{\sin \theta} \, \partial_{\phi} Y^m_l(\theta, \phi) \, \hat{\boldsymbol{\phi}} \right]
    \end{split}
    \label{eq:vsh}
\end{equation}
with $Y^m_l$ the spherical harmonics.
Note that the factor $1/r$ is taken out of the expansion to account for far field radiation. 
Furthermore, we note that with this field expansion we are now working in spherical coordinates $\boldsymbol{\mathbf{r}} = (r, \theta, \phi)$.
Each of these components can be found using the orthonormality relation of the vector spherical harmonics
\begin{equation}
    F_{lm}^{V}(r)= r \int \sin \theta d\theta \, d\phi ~ \boldsymbol{\mathbf{F}}(\boldsymbol{\mathbf{r}})\cdot\left[\boldsymbol{\mathbf{V}}_{l}^{m}\left(\theta,\phi\right)\right]^{*}.
    \label{eq:ortho_vsh}
\end{equation}
Inserting the expansion in Eq.~\eqref{eq:expansion} in Maxwell's equations (Eq.~(3) in the main text) gives an independent set of equations for each $\{l,m\}$ pair
\begin{equation}
    \begin{split}
        D_{lm}^{Y}(r) &= \frac{1}{\omega\mu_{0}} \left[\frac{\sqrt{l(l+1)}B_{lm}^{X}(r)}{r} - i\frac{dB_{lm}^{Z}(r)}{dr} \right] \\
        B_{lm}^{X}(r) &= \frac{\sqrt{l(l+1)} E_{lm}^{Y}(r)}{\omega r} \\
        B_{lm}^{Z}(r) &= \frac{-i}{\omega}\frac{dE_{lm}^{Y}(r)}{dr} \\
        B_{lm}^{Y}(r) &= -\frac{1}{\omega} \left[\frac{\sqrt{l(l+1)} E_{lm}^{X}(r)}{r} - i\frac{dE_{lm}^{Z}(r)}{dr} \right] \\
        D_{lm}^{X}(r) &= -\frac{\sqrt{l(l+1)} B_{lm}^{Y}(r)}{\omega\mu_{0}r} \\
        D_{lm}^{Z}(r) &= \frac{i}{\omega\mu_{0}}\frac{dB_{lm}^{Y}(r)}{dr}. \\
    \end{split} \label{eq:XYZrel}
\end{equation}
Outside the sphere the permittivity is isotropic and Maxwell's equations further split into two independent sets of equations, one for ${\{E_{lm}^{Y},B_{lm}^{X},B_{lm}^{Z}\}}$ and one for ${\{B_{lm}^{Y},E_{lm}^{X},E_{lm}^{Z}\}}$. 
Outside the sphere both $E_{lm}^{Y}(r)$ and $B_{lm}^{Y}(r)$, satisfy, 
\begin{equation}
\frac{d^{2}F}{dr^{2}}+\left(k_{0}^{2}-\frac{l(l+1)}{r^{2}}\right)F=0
\label{outside_sphere}
\end{equation}
with $k_{0}=\omega/c$. 
This expression has two independent solutions known as Riccati-Bessel functions, $S_{l}(k_{0}r)$ and $C_{l}(k_{0}r)$, which are related to the Bessel functions via
\begin{equation}
    \begin{split}
        S_{l}(x) &= \sqrt{\frac{\pi x}{2}}J_{\frac{l+1}{2}}(x), \\[0.1cm]
        C_{l}(x) &= -\sqrt{\frac{\pi x}{2}}Y_{\frac{l+1}{2}}(x).
    \end{split}
\end{equation}
While $S_{l}$ is finite everywhere, $C_{l}$ diverges at the origin. The linear combinations
\begin{equation}
    \begin{split}
        \xi_{l}(x) & =S_{l}(x) - iC_{l}(x) \\[0.1cm]
        \zeta_{l}(x) &= S_{l}(x) + iC_{l}(x)
    \end{split}
\end{equation}
as $x\rightarrow\infty$ satisfy the relations
\begin{equation}
    \begin{split}
        \xi_{l}(x) &\propto e^{+ ix}, \\[0.1cm]
        \zeta_{l}(x) &\propto e^{- ix}.
    \end{split}
\end{equation}
Consequently, they can be interpreted as outgoing and incoming waves.
Given $E_{lm}^{Y}$ and $B_{lm}^{Y}$, the other components can be found from Eqs.~(\ref{eq:XYZrel}). The two sets of eigensolutions are labelled as TE (transverse electric) and TM (transverse magnetic). They are given by,
\begin{equation}
\begin{split}
    \mathbf{E}_{lm,\text{TE}} &= \frac{R_l(k_0r)}{k_0r} \mathbf{Y}_l^m(\theta,\phi) \\
    \mathbf{E}_{lm,\text{TM}} &= \frac{c}{k_0r} \left[ -\sqrt{l(l+1)} \frac{R_l(k_0r)}{k_0r} \mathbf{X}_l^m(\theta,\phi) + iR'_l(k_0r) \mathbf{Z}_l^m(\theta,\phi) \right],
\end{split} \label{eq:eigens}
\end{equation}
where $R_l(k_0r)$ can be any linear combination of $S_l$ and $C_l$. The magnetic field is given by $\text{TE}\leftrightarrow\text{TM}$, $\mathbf{E}\rightarrow\mathbf{B}$, and $c\rightarrow -1/c$.


%Incidental fields
\subsection{Incident and scattered fields}
\label{sup:incident}

The incident field should be finite everywhere as it is generated by an external source far from the sphere, so it can be modelled as the linear combination given in Eq.~(4) of the main text,
\begin{equation}
    \mathbf{E}_{\text{in}}(\mathbf{r}) = \sum_{lm} \frac{1}{k_0r} \left[ \mathcal{E}_{lm}^{\text{in}} \mathbf{E}^{\text{in}}_{lm,\text{TE}} + c\mathcal{B}_{lm}^{\text{in}} \mathbf{E}^{\text{in}}_{lm,\text{TM}}  \right], \label{eq:expansion_in}
\end{equation}
for an arbitrary set of coefficients $\{\mathcal{E},\mathcal{B}\}$ and $\mathbf{E}^{\text{in}} = k_0r\mathbf{E}$ in terms of Eqs.~(\ref{eq:eigens}) with $R_l\rightarrow S_l$.

The scattered field is given by an analogous expansion with $\mathcal{E}^{\text{in}}\rightarrow \mathcal{E}^{\text{S}}$ and $R_l\rightarrow \xi_l$ to model outgoing waves.

%Mie fields
\subsection{Mie scattered fields}
\label{sup:mie}
When $f_{\text{F}}=0$, there is no Faraday rotation, and the problem reduces to Mie scattering. In the above notation, $\mathcal{E}_{lm}^{\text{S}} = \mathcal{E}_{lm}^{\text{M}}$.
In that case, the fields inside the sphere also satisfy Eq.~\eqref{outside_sphere} but with $k_{0}\rightarrow k=nk_{0}$ where $n$ is the refractive index. 
Thus, the fields inside the sphere ($r<R$) are given by an expansion analogous to Eq.~(\ref{eq:expansion_in}) with $\mathcal{E}^{\text{in}} \rightarrow \mathcal{E}^{\text{sp}}$ and $k_0\rightarrow k$. The coefficients can be found using the continuity of $\{D_{lm}^{X},E_{lm}^{Y},E_{lm}^{Z},B_{lm}^{X},B_{lm}^{Y},B_{lm}^{Z}\}$
for each $lm$ at the boundary. 
Explicitly,
\begin{equation}
    \begin{split}
        \mathcal{E}^{\text{sp}}_{l}S_{l}(n k_0 R) & =\mathcal{E}^{\text{in}}_{l}S_{l}(k_{0}R)+\mathcal{E}^{\text{M}}_{l}\xi_{l}(k_{0}R)\\
        k\mathcal{E}^{\text{sp}}_{l}S_{l}'(n k_0 R) & =k_{0}\mathcal{E}^{\text{in}}_{l}S_{l}'(k_{0}R)+k_{0}\mathcal{E}^{\text{M}}_{l}\xi_{l}'(k_{0}R)\\
        \mathcal{B}^{\text{sp}}_{l}S_{l}(n k_0 R) & =\mathcal{B}^{\text{in}}_{l}S_{l}(k_{0}R)+\mathcal{B}^{\text{M}}_{l}\xi_{l}(k_{0}R)\\
        \frac{k}{\epsilon}\mathcal{B}^{\text{sp}}_{l}S_{l}'(n k_0 R) & =\frac{k_{0}}{\epsilon_{0}}\mathcal{B}^{\text{in}}_{l}S_{l}'(k_{0}R)+\frac{k_{0}}{\epsilon_{0}}\mathcal{B}^{\text{M}}_{l}\xi_{l}'(k_{0}R).
\end{split}
\end{equation}
Using the identity $S_{l}(x)\xi_{l}'(x)-S_{l}'(x)\xi_{l}(x)=i$ the excitation amplitude turns out to be
\begin{equation}
    \begin{split}
        \frac{\mathcal{E}^{\text{sp}}_{l}}{\mathcal{E}^{\text{in}}_{l}} & =\frac{i}{S_{l}(n k_0 R)\xi_{l}'(k_{0}R)-nS_{l}'(n k_0 R)\xi_{l}(k_{0}R)}\triangleq\chi_{l}^{\text{E}} \label{Exc:TE}\\
        \frac{\mathcal{B}^{\text{sp}}_{l}}{\mathcal{B}^{\text{in}}_{l}} & =\frac{i}{S_{l}(n k_0 R)\xi_{l}'(k_{0}R)-n^{-1}S_{l}'(n k_0 R)\xi_{l}(k_{0}R)}\triangleq\chi_{l}^{\text{B}},
    \end{split}
\end{equation}
where $\chi$ can be interpreted as susceptibility.
The radiation amplitude of the Mie scattered field is given by
\begin{equation}
    \begin{split}
        \frac{\mathcal{E}^{\text{M}}_{l}}{\mathcal{E}^{\text{in}}_{l}} & =\frac{nS_{l}'(n k_0 R)S_{l}(k_{0}R)-S_{l}'(k_{0}R)S_{l}(n k_0 R)}{S_{l}(n k_0 R)\xi_{l}'(k_{0}R)-nS_{l}'(n k_0 R)\xi_{l}(k_{0}R)}\triangleq r_{l}^{\text{E}}\\
        \frac{\mathcal{B}^{\text{M}}_{l}}{\mathcal{B}^{\text{in}}_{l}} & =\frac{n^{-1}S_{l}'(n k_0 R)S_{l}(k_{0}R)-S_{l}'(k_{0}R)S_{l}(n k_0 R)}{S_{l}(n k_0 R)\xi_{l}'(k_{0}R)-n^{-1}S_{l}'(n k_0 R)\xi_{l}(k_{0}R)}\triangleq r_{l}^{\text{B}}.
        \label{rad_amp_mie}
    \end{split}
\end{equation}
We note that the polarization and the angular momentum are preserved in an isotropic scattering process. 

%Faraday fields
\subsection{Faraday scattered fields}
\label{sup:faraday}

When $f_{\text{F}} \ne 0$, the scattered light can be written as $\mathcal{E}_{lm}^{\text{S}} = \mathcal{E}_{lm}^{\text{M}} + \mathcal{E}_{lm}^{\text{F}}$, where $\mathcal{E}_{lm}^{\text{M}}$ was found in the previous subsection. For a sphere of radius $\SI{1}{\micro\meter}$ and typical Faraday rotation of $<1 \si{\deg/\micro\meter}$, the Faraday effect is a small perturbation. In this section, we find the leading order contribution to the scattered light due to Faraday rotation. As we show below, the Mie scattered component is largely unaffected except for a small renormalization of susceptibility $\chi$, and the Faraday effect inverts the polarization, i.e. we can write 
\begin{equation}
\begin{split} 
    \mathcal{B}_{lm}^{\text{F}} &= \frac{f_{\text{F}}}{c} \sum_L \mathcal{T}^{\text{B}}_{Llm} \mathcal{E}_{Lm}^{\text{in}} \\
    \mathcal{E}_{lm}^{\text{F}} &= f_{\text{F}}c \sum_L \mathcal{T}^{\text{E}}_{Llm} \mathcal{B}_{Lm}^{\text{in}}
\end{split} \label{def:Farcoeff}
\end{equation}
Note that the azimuthal index $m$ doesn't change due to azimuthal symmetry.

The electric field inside the sphere is given by $\mathbf{E} = \mathbf{E}_{\text{sp}} + \mathbf{E}_{\text{F}}$, where $\mathbf{E}_{\text{sp}}$ was calculated in the previous subsection and $\mathbf{E}_{\text{F}}\propto f_{\text{F}}$ is the linear correction due to the Faraday effect, to be calculated. The displacement vector is given by
\begin{equation}
    \mathbf{D} = \varepsilon_0 \left( \varepsilon_r \mathbf{E} + if_{\text{F}}\text{M}_{\text{s}} \mathbf{z}\times\mathbf{E} \right).
\end{equation}
For simplifying this further, we need the following identities
\begin{align}
    \mathbf{z}\times\mathbf{Y}_{l}^{m} &= -\frac{im}{l(l+1)}\mathbf{Y}_{l}^{m} + g_l^m\mathbf{Z}_{l-1}^{m} + g_{l+1}^m\mathbf{Z}_{l+1}^{m} - ig_l^m\sqrt{\frac{l}{l-1}}\mathbf{X}_{l-1}^{m} + ig_{l+1}^m\sqrt{\frac{l+1}{l+2}}\mathbf{X}_{l+1}^{m} \\
    \mathbf{z}\times\mathbf{X}_{l}^{m} &= -\frac{m}{\sqrt{l(l+1)}}\mathbf{Z}_{l}^{m} + ig_l^m\sqrt{\frac{l}{l+1}}\mathbf{Y}_{l-1}^{m} - ig_{l+1}^m\sqrt{\frac{l+1}{l}}\mathbf{Y}_{l+1}^{m} \\
    \mathbf{z}\times\mathbf{Z}_{l}^{m} &= -\frac{im}{l(l+1)}\mathbf{Z}_{l}^{m} - \frac{m}{\sqrt{l(l+1)}}\mathbf{X}_{l}^{m} - g_l^m\mathbf{Y}_{l-1}^{m} - g_{l+1}^m\mathbf{Y}_{l+1}^{m}.
\end{align}
Here,
\begin{equation}
    g_l^m = \sqrt{\frac{l^{2}-1}{l^{2}}\frac{l^{2}-m^{2}}{4l^{2}-1}}.
\end{equation}
These identities can be found using the known recursion relations of scalar spherical harmonics. 

\emph{TE-input:} Consider first a purely TE mode with angular momentum numbers $LM$, i.e. $\mathcal{B}_{lm}^{\text{in}} = 0$ and $\mathcal{E}_{lm}^{\text{in}} = \mathcal{E}\delta_{lL}\delta_{mM}$. For this case, we can write the VSH components of the displacement vector up to first order in $f_{\text{F}}$ as
\begin{align}
    D_{LM}^{Y} &\approx \epsilon_{s} \chi_{L}^{\text{E}}\ \text{E}_0S_{L}(kr) \left[ 1+\frac{if_{\text{F}}\text{M}_{\text{s}}}{L(L+1)} \right] + \varepsilon_0\varepsilon_r E_{F,LM}^{Y} \\
    D_{L-1,M}^{X} &\approx -\sqrt{\frac{L}{L-1}} \varepsilon_0\varepsilon_r \mathcal{I}_- S_{L}(kr) + \varepsilon_0\varepsilon_r E_{F,L-1,M}^{X} \\
    D_{L-1,M}^{Z} &\approx -i\varepsilon_0\varepsilon_r {\cal I}_{-} S_{L}(kr) + \varepsilon_0\varepsilon_r E_{F,L-1,M}^{Z} \\
    D_{L+1,M}^{X} &\approx \sqrt{\frac{L+1}{L+2}} \varepsilon_0\varepsilon_r {\cal I}_+ S_{L}(kr) + \varepsilon_0\varepsilon_r E_{F,L+1,M}^{X} \\
    D_{L+1,M}^{Z} &\approx -i\varepsilon_0\varepsilon_r {\cal I}_{+} S_{L}(kr) + \varepsilon_0\varepsilon_r E_{F,L+1,M}^{Z},
\end{align}
where ${\cal I}_{+} = g_{L+1}^M f_{\text{F}} \text{M}_{\text{s}} \chi_{L}^{\text{E}} {\cal E}$, and ${\cal I}_{-} = g_{L}^M f_{\text{F}} \text{M}_{\text{s}} \chi_{L}^{\text{E}}{\cal E}$. All the other coefficients are higher order in $f_{\text{F}}$. The corrections to $D^Y$ cause a small renormalization of the Mie frequency and can be ignored. 

We insert the above into the last three Maxwell's equations, Eqs.~\ref{eq:XYZrel}, and eliminate $E_F^X$ and $E_F^Z$ to get an equation for $B_F^Y$,
\begin{equation}
    \frac{d^{2} B_{F,L\pm1,M}^{Y}(r)}{k^{2}dr^{2}} + \left( 1 - \frac{(L\pm1+1)(L\pm1)}{k^{2}r^{2}} \right) B_{F,L\pm1,M}^{Y}(r) = \pm\frac{n {\cal I}_{\pm}}{c} S_{L\pm1}(kr),
\end{equation}
where we used the recursion relations for Riccati-Bessel functions
\begin{align}
    S_{l-1}(x) &= S_{l}'(x) + \frac{lS_{l}(x)}{x} \\
    S_{l+1}(x) &=-S_{l}'(x) + \frac{(l+1)S_{l}(x)}{x}.
\end{align}
The general solution of this differential equation is
\begin{equation}
    b_{L\pm1}^{Y}(r) = \pm\frac{n{\cal I}_{\pm}}{c} \left[p_{L\pm1}(kr)+\alpha_{\pm}S_{L\pm1}(kr)\right],
\end{equation}
where $\alpha_{\pm}$ are unknown constants and $p_{l}(x)$ is any solution satisfying
\begin{equation}
    \frac{d^{2}p_{l}}{dx^{2}}+\left(1-\frac{l(l+1)}{x^{2}}\right)p_{l}=S_{l}(x)
\end{equation}
and $p_{l}(0)=0$. While it is possible to write an explicit formula for $p_{l}$, below we need only the Wronskian $W_{l}=p_{l}'S_{l}-p_{l}S_{l}'$ which satisfies 
\begin{equation} 
W_{l}'(x)=S_{l}^{2}(x) \Rightarrow W_{l}(x) = \frac{x}{2} \left[S_{l}^{2}(x)-S_{l+1}(x)S_{l-1}(x)\right],
\end{equation}
where $p_{l}(0)=S_{l}(0)=0$ is used.

So far, we found that the electromagnetic fields inside the sphere have a large component in $\{LM,\text{TE}\}$ and small Faraday scattered components in $\{L\pm1,M,\text{TM}\}$. Via the boundary conditions, this will also hold outside the sphere, so we can write the scattered light as $\mathcal{E}_{lm} = r_L^{\text{E}} \text{E}_0\delta_{lL}\delta_{mM}$ and
\begin{equation}
    c\mathcal{B}^{\text{F}}_{lm} = f_{\text{F}}\mathcal{E}\left(P_{LM}^{\text{B}}\delta_{l(L+1)}\delta_{mM}+M_{LM}^{\text{B}}\delta_{l(L-1)}\delta_{mM}\right).
\end{equation}
We can find these coefficients by the boundary conditions that turn out to be
\begin{align}
    p_{L\pm1}(kR) + \alpha_{\pm} S_{L\pm1}(kR) &= \frac{\pm c\mathcal{B}^{\text{F}}_{L\pm1,M}}{n{\cal I}_{\pm}} \xi_{L\pm1}(k_{0}R) \\
    p'_{L\pm1}(kR) + \alpha_{\pm} S_{L\pm1}'(kR)\pm S_{L}(kR) &= \frac{\pm c\mathcal{B}^{\text{F}}_{L\pm1,M}}{{\cal I}_{\pm}} \xi_{L\pm1}'(k_{0}R).
\end{align}
These give
\begin{align}
    P^{\text{B}}_{lm} &= -i\chi_l^{\text{E}} \chi_{l+1}^{\text{B}} g_{l+1}^m \left[ W_{l+1}(kR) + S_l(kR)S_{l+1}(kR)\right] \\
    M^{\text{B}}_{lm} &= i\chi_l^{\text{E}} \chi_{l-1}^{\text{B}} g_l^m \left[ W_{l-1}(kR) - S_l(kR)S_{l-1}(kR)\right]
\end{align}

As the calculations for the TM input are analogous, we simply write down the final result here. We define similar coefficients as above,\begin{align}
    P^{\text{E}}_{lm} &= -i\chi_l^{\text{B}} \chi_{l+1}^{\text{E}} g_{l+1}^m W_{l+1}(kR) \\
    M^{\text{E}}_{lm} &= i\chi_l^{\text{B}} \chi_{l-1}^{\text{E}} g_l^m W_{l-1}(kR).
\end{align}

Then, the scattering coefficients in the notation of Eqs.~(\ref{def:Farcoeff}) are
\begin{equation}
    {\cal T}^{\sigma}_{Llm} = P_{LM}^{\sigma} \delta_{l(L+1)}\delta_{mM} + M_{LM}^{\sigma} \delta_{l(L-1)}\delta_{mM}
\end{equation}

For a plane wave, $\text{E}_0 \, e^{ik_0z} \hat{\mathbf{x}}$, we have the input~\cite{mie}
\begin{align}
    \mathcal{E}^{\text{in}}_{lm} &= \text{E}_0\sqrt{\pi(2l+1)} i^l \left(\delta_{m,1} + \delta_{m,-1}\right) \\
    \mathcal{B}^{\text{in}}_{lm} &= \frac{\mathcal{E}}{c} \sqrt{\pi(2l+1)} i^{l+1} \left(\delta_{m,1} - \delta_{m,-1}\right)
\end{align}

Then, the expressions for Mie and the Faraday scattered light, as written in the main text, directly follow.


\section{Effective permittivity tensor of magnetic materials}
For capturing the Faraday effect mathematically we derive the modified effective permittivity tensor.
We can always expand the displacement vector as
\begin{equation}
    \mathbf{D} = f_\text{E}\mathbf{E} + f_{\text{M}}\mathbf{M} + f_{\times} \mathbf{M}\times\mathbf{E},
\end{equation}
where $f$ are functions of $\mathbf{E}$ and $\mathbf{M}$. 
As the system is rotationally symmetric, all of $f$ should be a function of only $|\mathbf{E}|^2$ and $\mathbf{E}\cdot\mathbf{M}$ as $|\mathbf{M}|^2$ is a constant.
Assuming that there are no non-linear optical processes, which are weak in typical materials, we need to keep only the terms that are linear in $\mathbf{E}$. Then, the most general form is
\begin{equation}
    \mathbf{D} = \varepsilon_0 \left( \varepsilon_r \mathbf{E} + f_C \mathbf{M}\cdot\mathbf{E}\  \mathbf{M} + if_{\text{F}} \mathbf{M}\times\mathbf{E} \right),
\end{equation}
with constants $\{\varepsilon_r,f_{\text{C}},f_{\text{F}}\}$. As the permittivity should be Hermitian, all of these constants are real.

For simplicity, we ignore the Cotton-Mouton effect ($\propto f_C$). Then, we get
\begin{equation}
    \varepsilon_{ik}(\boldsymbol{\mathbf{M}}) = \varepsilon_0 \bigg( \varepsilon_r \delta_{ik} - i f_{\text{F}} \sum_j \varepsilon_{ikj} M_j \bigg).
\label{permittivity_faraday}
\end{equation} 
For including also dispersive magnetic materials the relative permittivity and the Faraday constant need to be made frequency dependent by using appropriate models for $\varepsilon_r(\omega)$ and $f_{\text{F}}(\omega)$ (see Eq.~(26) in the main text).

\section{Extension of the FDTD method to dispersive magnetic materials}
Below we provide additional derivations used for extending the FDTD method to dispersive magnetic dielectrics.

\subsection{Fourier transforms}
For transforming the optical response in the frequency domain into the time domain using a Fourier transformation, the following substitutions need to be made
\begin{equation}
    \begin{split}
        - i\omega &\rightarrow \partial_t, ~~~~~~~~~~ - \omega^2 \rightarrow \partial_t^2, \\[0.2cm]
        i \omega^3 &\rightarrow \partial_t^3, ~~~~~~~~~~~~  \omega^4 \rightarrow \partial_t^4.
    \end{split}
\end{equation}

\subsection{Update equations for the polarization vector}
For deriving the update equation for the polarization vector we need to discretize Eq.~(28) in the main text using central differencing.
By centering the central differences at time step $n-1$, the update equations for the polarization are
\begin{equation}
    \begin{split}
        \left( \frac{1}{\boldsymbol{\triangle} t^4} + \frac{\eta}{\boldsymbol{\triangle}t^3} \right) \boldsymbol{\mathbf{P}}^{n+1}
        &= \left( \frac{4}{\boldsymbol{\triangle}t^4} + \frac{2 \eta}{\boldsymbol{\triangle}t^3} - \frac{2 \omega_0^2 + \eta^2}{\boldsymbol{\triangle}t^2} - \frac{\omega_0^2 \eta}{\boldsymbol{\triangle}t}  \right) \boldsymbol{\mathbf{P}}^n + \left( -\omega_0^4 - \frac{6}{\boldsymbol{\triangle}t^4} + 2 \frac{2 \omega_0^2 + \eta^2}{\boldsymbol{\triangle}t^2} \right) \boldsymbol{\mathbf{P}}^{n-1} \\[0.2cm]
        &+ \left( \frac{4}{\boldsymbol{\triangle}t^4} - \frac{2 \eta}{\boldsymbol{\triangle}t^3} - \frac{2 \omega_0^2 + \eta}{\boldsymbol{\triangle}t^2} \frac{\omega_0^2 \eta}{\boldsymbol{\triangle}t} \right) \boldsymbol{\mathbf{P}}^{n-2} + \left( - \frac{1}{\boldsymbol{\triangle}t^4} + \frac{\eta}{\boldsymbol{\triangle}t^3} \right) \boldsymbol{\mathbf{P}}^{n-3} \\[0.2cm]
        & + \omega_0^2 \varepsilon_0 (\varepsilon -1 ) \Big[ \left( \frac{1}{\boldsymbol{\triangle}t^2} + \frac{\eta}{2\boldsymbol{\triangle}t} \right) \boldsymbol{\mathbf{E}}^n  + \left( \omega_0^2 - \frac{2}{\boldsymbol{\triangle}t^2} \right) \boldsymbol{\mathbf{E}}_{n-1}\\[0.2cm]
        &  + \left( \frac{1}{\boldsymbol{\triangle}t^2} - \frac{\eta}{2 \boldsymbol{\triangle}t} \right) \boldsymbol{\mathbf{E}}^{n-1} \Big] - \frac{\varepsilon_0 A_3 \omega_0}{2 \boldsymbol{\triangle} t} \, \boldsymbol{\boldsymbol{\mathbf{M}}} \times \left( \boldsymbol{\mathbf{E}}^n - \boldsymbol{\mathbf{E}}^{n-2} \right)
    \end{split}
\end{equation}
which then include the magnetic model into the update equations via the electric field
\begin{equation}
    \boldsymbol{\mathbf{E}}^{n+1} = \boldsymbol{\mathbf{E}}^{n} + \frac{\boldsymbol{\triangle} t}{\varepsilon_0} \, \nabla \times \boldsymbol{\mathbf{H}}^{n+1/2} - \frac{1}{\varepsilon_0} \left( \boldsymbol{\mathbf{P}}^{n+1} - \boldsymbol{\mathbf{P}}^n \right).
\end{equation}
Thus, for any given time step, we need to store $\boldsymbol{\mathbf{E}}^{n+1}$, $\boldsymbol{\mathbf{E}}^n$, $\boldsymbol{\mathbf{E}}^{n-1}$, $\boldsymbol{\mathbf{E}}^{n-2}$, $\boldsymbol{\mathbf{P}}^{n+1}$, $\boldsymbol{\mathbf{P}}^n$, $\boldsymbol{\mathbf{P}}^{n-1}$, $\boldsymbol{\mathbf{P}}^{n-2}$, and $\boldsymbol{\mathbf{P}}^{n-3}$.

%##############################################################

% \bigvbliography{main}
% \end{document}
